AI-Driven Container Security Approaches for 5G and Beyond: A Survey

The rising use of microservices based software deployment on the cloud leverages containerized software extensively. The security of applications running inside containers as well as the container environment itself are critical infrastructure in the cloud setting and 5G. To address the security concerns, research efforts have been focused on container security with subfields such as intrusion detection, malware detection and container placement strategies. These security efforts are roughly divided into two categories: rule based approaches and machine learning that can respond to novel threats. In this study, we have surveyed the container security literature focusing on approaches that leverage machine learning to address security challenges.

==> attack_detection_table.tex <==
\begin{table*}[ht]
    \begin{center}
        \caption{Overview of surveyed attack detection in container approaches}%
        \label{tab:attack-detection}
        \begin{small}
            \begin{tabularx}{\linewidth}{@{} t g m m b @{}}
                \toprule
                \thead{Work} & \thead{Method\\Used} & \thead{Monitoring} & \thead{Feature\\Extraction} & \thead{Detected\\Attacks}\\
                \midrule
                \cite{linSHIL2022} & Autoencoder & Sysdig, JMeter & BoSC & return a shell and arbitrary code execution \\
                \cite{linCDL2020}  & Random Forest & Sysdig, JMeter & BoSC & arbitrary code execution, disclose credential info, consume excessive CPU, privilege escalation \\
                \bottomrule
            \end{tabularx}
        \end{small}
    \end{center}
\end{table*}


==> inter_container_security_table.tex <==
\begin{table*}[ht]
    \begin{center}
        \caption{Overview of inter container security in container approaches}%
        \label{tab:inter-container-security}
        \begin{small}
            \begin{tabularx}{\linewidth}{@{} t b b b @{}}
                \toprule
                \thead{Work} & \thead{ML\\Method} & \thead{Attacks} & \thead{Motivation} \\
                \midrule
                \cite{dengSecure2022} & DRL & Co-resident attack & Container placement \\
                \cite{liOptimal2022} & DRL & Random-walker attacker, persistent attacker & Decoy placement \\
                \cite{kongSecure2019} & Genetic algorithm & Co-resident attack & Container placement \\
                \bottomrule
            \end{tabularx}
        \end{small}
    \end{center}
\end{table*}


==> malware_detection_table.tex <==
\begin{table*}[ht]
    \begin{center}
        \caption{Overview of surveyed malware detection in container approaches}%
        \label{tab:malware-detection}
        \begin{small}
            \begin{tabularx}{\linewidth}{@{} t b b b b @{}}
                \toprule
                \thead{Work} & \thead{ML\\Method} & \thead{Feature\\Extraction} & \thead{Dataset} & \thead{Attack} \\
                \midrule
                \cite{wangDockerWatch2022} & LSTM, CNN & Disassembled bytecode section info of ELF, n-gram frequency of opcode & 300 attack exploits + 2000 benign and 3000 malicious ELF binaries & privilege escalation, container info leakeage \\
                \cite{karnCryptomining2021} & Decision Tree, Ensemble learning, Feed-forward vanilla NN, Feedback RNN & n-grams & %% TODO is it ok? or too long
                System call length for pods: 2.038.829 Bitcoin, 481466 Bytecoin, 28850 Vertcoin, 61634 Dashcoin, 290657 Litecoin, 77981 Deeplearning, 14756 Mysql, 910472 Cassandra, 1656599 Hadoop, 270981 Graph & cryptojacking, malware \\
                \bottomrule
            \end{tabularx}
        \end{small}
    \end{center}
\end{table*}

